Discovering Fatigued Movements for Virtual Character Animation

Virtual character animation and movement synthesis have advanced rapidly during recent years, especially through a combination of extensive motion capture datasets and machine learning. A remaining challenge is interactively simulating characters that fatigue when performing extended motions, which is indispensable for the realism of generated animations. However, capturing such movements is problematic, as performing movements like backflips with fatigued variations up to exhaustion raises capture cost and risk of injury. Surprisingly, little research has been done on faithful fatigue modeling. To address this, we propose a deep reinforcement learning-based approach, which -- for the first time in literature -- generates control policies for full-body physically simulated agents aware of cumulative fatigue. For this, we first leverage Generative Adversarial Imitation Learning (GAIL) to learn an expert policy for the skill; Second, we learn a fatigue policy by limiting the generated constant torque bounds based on endurance time to non-linear, state- and time-dependent limits in the joint-actuation space using a Three-Compartment Controller (3CC) model. Our results demonstrate that agents can adapt to different fatigue and rest rates interactively, and discover realistic recovery strategies without the need for any captured data of fatigued movement.

==> fig/fig_overview.tex <==
\begin{figure}
	\includegraphics[width=\linewidth]{img/SA_overview_compressed.png}
	\caption
	{\textbf{Overview.} Our framework consists of two stages: A pre-training stage where the policy learns to imitate the motion clip.
    Then a transfer learning stage, where an adaptive fatigue policy is learned by constraining the output torques of the PD-controllers based on the computed torque bounds by the Residual Capacity ($RC$) from the 3CC-model.
    }
	%
	\label{fig:overview}
	%
\end{figure}

==> fig/fig_teaser.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}
    \includegraphics[width=\linewidth]{img/SA_fitness_control.png}
	%
	\caption
	{
    %
    We propose a deep reinforcement learning approach, which explicitly accounts for a character's fatigue.
    %
    We show that our agents discover novel fatigued motions and recovery strategies without requiring explicit fatigued data.
    %
    Moreover, our approach enables interactive fitness control within one policy, letting characters fatigue faster or slower depending on the user.
    %
	}
	%
	\label{fig:teaser}
	%
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
